SynCity: Training-Free Generation of 3D Worlds

We address the challenge of generating 3D worlds from textual descriptions. We propose SynCity, a training- and optimization-free approach, which leverages the geometric precision of pre-trained 3D generative models and the artistic versatility of 2D image generators to create large, high-quality 3D spaces. While most 3D generative models are object-centric and cannot generate large-scale worlds, we show how 3D and 2D generators can be combined to generate ever-expanding scenes. Through a tile-based approach, we allow fine-grained control over the layout and the appearance of scenes. The world is generated tile-by-tile, and each new tile is generated within its world-context and then fused with the scene. SynCity generates compelling and immersive scenes that are rich in detail and diversity.

==> figures/denoise3d-fig.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.85\textwidth]{images/denoise-3d.jpg}
\caption{\textbf{Denoising the stitch region in 3D} {\color{red} Suny: I will improve the figure. The blue region should be ``noise'' and is what is denoised.}}
\label{fig:denoise3d}
\end{figure*}
